Optimisation of cyber insurance coverage with selection of cost effective security controls

Nowadays, cyber threats are considered among the most dangerous risks by top management of enterprises. One way to deal with these risks is to insure them, but cyber insurance is still quite expensive. The insurance fee can be reduced if organisations improve their cyber security protection, i.e., reducing the insured risk. In other words, organisations need an investment strategy to decide the optimal amount of investments into cyber insurance and self-protection. In this work, we propose an approach to help a risk-averse organisation to distribute its cyber security investments in a cost-efficient way. What makes our approach unique is that next to defining the amount of investments in cyber insurance and self-protection, our proposal also explicitly defines how these investments should be spent by selecting the most cost-efficient security controls. Moreover, we provide an exact algorithm for the control selection problem considering several threats at the same time and compare this algorithm with other approximate algorithmic solutions.

==> 00_Rebuttal.tex <==
\section{Update and comments}


\newcounter{reviewer}
%\setcounter{reviewer}{1}
\newcounter{comment}[reviewer]
\def\reviewer{\refstepcounter{reviewer}\section*{\textsf{Comments from Reviewer 2 }}}
\def\comment{\refstepcounter{comment}\subsection*{\textsf{Comment }\thecomment}}
\def\reply{\subsubsection*{\textsc{Reply}}}

\def\reviewnote#1{\marginpar{#1}}
\long\def\fixed#1{{\color{red}#1}}
% Uncomment for submission
%\def\reviewnote#1{}
%\long\def\fixed#1{#1}

\reviewer \label{r1}
\comment \label{r1:goal1}
Intuitively, it seems that the initial model in Equation 1 is too complex, for the initial wealth of the company $ W_0 $ is a constant, and the total wealth "after security" is not changed but through the security expenditure. Perhaps, the model from Equation (1) would be more interesting in a game-theoretic setting, but as a simple one-step optimisation problem it looks like an over-complication.


\reply{1}
-	A.
\reply{2}
- B.
\reply{3} -	C.

\comment \label{r1:goal2}
As a suggestion, I would propose to rewrite Section 3.1, to focus on the minimal relevant model (Equations 2, 4, 9), which is basically an optimisation model for a company to minimise security investment. Then, a separate section can be dedicated to an extended model that considers insurance and wealth. In this new section, it can be shown that even in the presence of cyber insurance, the core optimisation model does not change (under the stated assumptions). The restructured presentation will help the reader to understand better the core ideas behind the paper.



\comment \label{r1:goal3}
It seems that the assumptions behind the model are quite strong (the insurer sets the premium at the actual risk level, what leads to the property of the model that a reasonable organisation will want to insure all risks that cannot be reduced). Are these assumptions realistic? It is known that currently some underwriters underprice cyber insurance, and also a company may decide to be slightly more risk tolerant, because dealing with a complex cyber insurance structure needed to completely insure all risks will incur additional costs.

\comment \label{r1:goal4}
Total insurance costs for an organisation are typically higher than what the insurer charges, because the organisation needs to spend time and money on managing the insurance (possible fees to a broker, insurance process preparation and set-up, etc.). Countermeasure independence, both in terms of threat resilience and costs, is also a very strong assumption that will not hold in practice (e.g., a SIEM event monitoring relies on an identity management solution in place, thus their effectiveness against threats is not independent). Finally, the approach assumes that for all considered controls it is possible to estimate a probability for each considered threat scenario occurring with this control implemented. It seems thus that the time investment for an organisation to bootstrap this cost-efficient countermeasure selection process is quite high. It is stated in Section 5.5 that a company "[...] is most likely to consider a much smaller number of possible controls and be more
focused on a small number of relevant threats [...]" If this would be the case, I am not sure if there is much value in the algorithms proposed, because an exhaustive search implemented in a spreadsheet would work perfectly fine for very small scenarios. So it is larger scenarios that are most interesting for organisations, because then it is hard for them to estimate things quickly.

\comment \label{r1:goal5}
A discussion that would systematically review the assumptions, assess what are their practical limitations, and propose some possible alleviations as future research avenues is needed.

\comment \label{r1:goal6}
Recent SoK paper on cyber insurance in IEEE S\&P 2020 should be included in the literature review (Dambra, Bilge \& Balzarotti "SoK: Cyber Insurance - Technical Challenges and a System Security Roadmap")


\comment \label{r1:goal7}
Page 4, lines 25-26: "[...] often starting with a basic knapsack problems [17] but also considering specific variation" - please consider rephrasing this sentence, as it is not clear what "specific variation" refers to. Is it "a variation of a knapsack problem"? Is it always the same variation for all cited literature here, or different variations?

\comment \label{r1:goal8}
The basic variables $ x $, $ P $ and $ Loss $ are introduced twice, first on page 5, then on page 6.

\comment \label{r1:goal9}
Page 7, line 31: It is not clear, why we are talking about a successful penetration into a system here, because cyber threats can be of different nature. More generically, this can be a probability that the threat scenario occurs given countermeasures in place. Also, it is not really clear at this point, why we are speaking here (and in Eq. 4) about the optimal solution $ K_s|x $, and not a generic set $ K_s $.


\comment \label{r1:goal10}
Page 8, Equation 5: It is not clear, why both $ F $ and $ Z $ are used in this equation. $ F $ is already a set of threat scenario frequencies that is expected by an organization (I presume, over a specific period of time). Why there is another variable $ z $ that also represents an amount of threats over a period of time (i.e., possible frequencies). According to line 46 on page 7, $ F $ is expected threat frequencies, because this is what the insurer wants to consider. Why there is a need to consider all possible threat scenario occurrences if there is already expected threat frequencies available?

\comment \label{r1:goal11}
Also, I cannot interpret the index $ i $ in $ p_i $ in Equation 5. What does it range over? I note that this index is present also in Eq. 6, but it is gone in Eq.7 when the expectation is computed.

\comment \label{r1:goal12}
Page 8, the final sentence of Section 3.1 is not clear to me. Which "models described above [...] are found to be valid" are referred to here? Models in this section, or in the related literature?

\comment \label{r1:goal13}
Figure 5 is hard to read in a printed copy. I would suggest to increase the font size.

\comment \label{r1:goal14}
Some references have a strange style for authors' names: "Surname\_1, Name\_1, Name\_2 Surname\_2, and Name\_3 Surname\_3". E.g., [4, 5, 6, 10], etc.


\comment \label{r1:goal15}
Typos\\
Page 4, line 26: The word "problems" appears twice. It should be "problem" in fact, and there is no space before the reference [17].
Page 4, lines 47-48: "[...] we propose our exact algorithmic solution [...] and adapted it for [...]" - some issue with tenses here.
Page 6, line 46: "that" is not needed here.
Page 16, line 16: "[...] used optimisation solutions [...]" - perhaps, "optimisation techniques/approaches" is better here.
Page 16, line 49: "[...] and check if" - should be "checks".
Page 18, line 10: "Windows 10 operational system" - should be "operating system".

\newcounter{reviewer1}
%\setcounter{reviewer}{1}
%\newcounter{comment}[reviewer]
\def\reviewer{\refstepcounter{reviewer1}\section*{\textsf{Comments from Reviewer 4 }}}
\def\comment{\refstepcounter{comment}\subsection*{\textsf{Comment }\thecomment}}
\def\reply{\subsubsection*{\textsc{Reply}}}




\reviewer \label{r2}
\comment \label{r2:goal1}
The text is well written. There are a few points to correct as punctuation.

\comment \label{r2:goal2}
The general goal can be more detailed to include how the goal will be achieved.

\comment \label{r2:goal3}
The related work and other references are actual and I'm not capable to perceive some omission. The authors made discussions about them and comparisons with the proposed work.

//////////////////////end////////////////

% In the preamble
%%%%%%%%%%%%%%%%%%%
\def\boxedreviewnote#1{\fbox{#1}}

\usepackage{xcolor}

\definecolor{darkred}{rgb}{0.8,0,0}

% Comment the following to get version without comments

\newcommand{\fixed}[1]{{\color{darkred}#1}}

\def\reviewnote#1{\marginpar{#1}}


\newcounter{reviewer}

\renewcommand{\thereviewer}{\Alph{reviewer}}

\newcounter{comment}[reviewer]

\def\editor{\section*{\dotfill\textsc{Comments from Meta-review }\dotfill}}

\def\reviewer{\refstepcounter{reviewer}\section*{\dotfill\textsc{Comments from Reviewer }\thereviewer\dotfill}}

\def\comment{\refstepcounter{comment}\subsection*{\textsc{Comment} \thereviewer.\thecomment}\ignorespaces}%\vspace{-0.5\baselineskip}}

%\def\reply{\vspace{-0.5\baselineskip}\subsubsection*{\textbf{Reply}}}

\def\reply{\vspace{0.5\baselineskip}\par\noindent\textbf{Reply:}\ignorespaces~\hangindent 7ex}

\def\newreply{\vspace{0.5\baselineskip}\par\noindent\hspace*{6ex}\ignorespaces~\hangindent 7ex}

%\vspace{-0.5\baselineskip}}

%\def\added{\textsc{\bf{Added text:}}\\}

%%%%%%%%%%%%%%%%%%%%%%

%\let\mylabel\label

%\def\label#1{\protect\expandafter\mylabel{#1}\protect\fbox{#1}}

%%%%%%%%%%%%%%%%%%%%%%%%



%%%%% In the text




%%%%%%%%%%%%%%%%%%%%%%%

\reviewer \label{r1}

\comment This paper focuses on formalizing existing knowledge of

the visible process of data sharing into a logical framework.

They provide a calculus based on intuitionistic quantifier-free

first-order logic which also contains custom inference rules regarding

known tracking behavior. Such an approach can be used by different

websites and advertisers to identify whether they need to comply

with relevant privacy regulations regarding PII collection. In

addition, one can verify different claims about tracking behavior

through the use of automated theorem provers. The authors also use

their logical framework to evaluate the effectiveness of different

privacy-enhancing technologies that are able to mitigate unintended

user tracking in the Alexa Top 100 websites based on data obtained

from the openWPM dataset.



Strengths:

\begin{compactitem}
	
	\item The paper is in general well written and easy to follow. It also does a commendable job in being self-contained regarding different aspects of the problem and their techniques.
	
	\item The formal part of the work performed by the authors is solid and makes sense.
	
	\item An impressive amount of work has gone into this paper.
	
	\item The authors have done a commendable job in scoping the problem in the sense that it is clear what is included in their formal model and what is excluded. 
	
\end{compactitem}



Weaknesses:

\begin{compactitem}
	
	\item The main criticism I have about the work is that the authors did not
	
	do a thorough job in motivating the problem and discussing different
	
	aspects of the problem in details (e.g., intended users, usability,
	
	extension, scalability, generality).
	
\end{compactitem}



\reply Thank you for your comments. We hope we have addressed your concerns

as we detail in the following answers.



\comment \label{r1:update:motivation}

The authors did not sufficiently motivate the need for formalizing the

known tracking behavior of the Internet. It seems the authors are formalizing

what is already known in the literature. What is the added value of this

formalisms? Are there atomic, ground predicates the framework can derive

which is hard to derive manually? Did the authors find such surprising

results? Is transitivity of data sharing the only sort of complications

in inferring facts? For instance, if x shares data with A, A then shares

it with B, and B then shares it with C, then one can derive that x's data

can be possessed by C.





\reply We indeed formalized the current techniques employed for tracking (as our goal is not to develop a new detection mechanism or analyze new techniques as showed in Tab.~\ref{tab:PaperComparison}).



\newreply The added value of the formalization stays in the ability to provide an explanation, in the form of a proof, to show tracking practices and that can help users in determine e.g. the adds-on to install or if certain websites should comply to COPPA due to interaction with children-related websites. We have added a paragraph (\emph{Goal}) in Section\S\ref{sec:introduction} to underline the added value of this framework. We further discussed the added value in an appropriate section (Section\S\ref{sec:scalability}).



\comment \label{r1:update:utility}

The possible utilities of their framework are scattered all

over the paper. I sincerely think that having it one place could drive

home the point easily. Also, such interesting and non-trivial finding

could motivate the use of such a framework.





==> 00_Reply.tex <==
% In the preamble
%%%%%%%%%%%%%%%%%%%
\def\boxedreviewnote#1{\fbox{#1}}



\definecolor{darkred}{rgb}{0.8,0,0}

% Comment the following to get a version without comments

\newcommand{\fixed}[1]{{\color{darkred}#1}}

\def\reviewnote#1{\marginpar{#1}}

{\Large\textbf{Response to the comments from the reviewers on the submitted paper}\dotfill} \\
%\dotfill\textsc{Response to the comments from the reviewers on the submitted paper}\dotfill}

We thank the reviewers for their constructive comments and valuable time. We have addressed all comments and modified the paper accordingly. Our detailed answers follow. 

Please note that all added corrections to the original manuscript are indicated in \textcolor{red}{red}. The second round comments are highlighted as \textcolor{blue}{blue}. 

\newcounter{reviewer}

\renewcommand{\thereviewer}{\Alph{reviewer}}

\newcounter{comment}[reviewer]

\def\editor{\section*{\dotfill\textsc{Comments from Meta-review }\dotfill}}

\def\reviewer{\refstepcounter{reviewer}\section*{\dotfill\textsc{Comments from Reviewer }\thereviewer\dotfill}}

\def\comment{\refstepcounter{comment}\subsection*{\textsc{Comment} \thereviewer.\thecomment}\ignorespaces}%\vspace{-0.5\baselineskip}}

%\def\reply{\vspace{-0.5\baselineskip}\subsubsection*{\textbf{Reply}}}

\def\reply{\vspace{0.5\baselineskip}\par\noindent\textbf{Reply:}\ignorespaces~\hangindent 7ex}

\def\newreply{\vspace{0.5\baselineskip}\par\noindent\hspace*{6ex}\ignorespaces~\hangindent 7ex}

%\vspace{-0.5\baselineskip}}

%\def\added{\textsc{\bf{Added text:}}\\}

%%%%%%%%%%%%%%%%%%%%%%

%\let\mylabel\label

%\def\label#1{\protect\expandafter\mylabel{#1}\protect\fbox{#1}}

%%%%%%%%%%%%%%%%%%%%%%%%



%%%%% In the text




%%%%%%%%%%%%%%%%%%%%%%%

\reviewer 

\comment Intuitively, it seems that the initial model in Equation 1 is too complex, for the initial wealth of the company $ W_0 $ is a constant, and the total wealth "after security" is not changed but through the security expenditure. Perhaps, the model from Equation (1) would be more interesting in a game-theoretic setting, but as a simple one-step optimisation problem it looks like an over-complication.

\reply We agree with the raised problem. Since the change will not affect the result of this work, we have changed random variables (expected wealth and losses) to problem's parameters i.e. constants. Moreover, the overall flow has been simplified as suggested by comment A.2. Section 3 has been restructured to address this (and the next) comment. 
%\newreply 

\comment As a suggestion, I would propose to rewrite Section 3.1, to focus on the minimal relevant model (Equations 2, 4, 9), which is basically an optimisation model for a company to minimise security investment. Then, a separate section can be dedicated to an extended model that considers insurance and wealth. In this new section, it can be shown that even in the presence of cyber insurance, the core optimisation model does not change (under the stated assumptions). The restructured presentation will help the reader to understand better the core ideas behind the paper.


\reply We are grateful for the suggestion. Section 3 has been restructured according to the reviewer's suggestion. In particular, we start with sub-section 3.1. "\emph{Security optimisation. No insurance case}" to introduce the basic concepts and introduce cyber insurance case in the following section, gradually adding more complex features (e.g., utility model) to the already defined scenario.

\comment It seems that the assumptions behind the model are quite strong (the insurer sets the premium at the actual risk level, what leads to the property of the model that a reasonable organisation will want to insure all risks that cannot be reduced). Are these assumptions realistic? It is known that currently some underwriters underprice cyber insurance, and also a company may decide to be slightly more risk tolerant, because dealing with a complex cyber insurance structure needed to completely insure all risks will incur additional costs. Total insurance costs for an organisation are typically higher than what the insurer charges, because the organisation needs to spend time and money on managing the insurance (possible fees to a broker, insurance process preparation and set-up, etc.). 

\reply The above-mentioned comments are covered in a new Section~\ref{sec:MAinDiscussion} where
we explicitly discuss the limitations of our theoretical basis and underline the made assumptions. The relevant text from the section is shown below:
\begin{quotation}
	\footnotesize
	\newreply Our solution is based on the competitive insurance market model, which is simple and widely used in theoretical insurance studies \cite{Rothschild, Akerlof}. This model allows us to focus on the core problems and simplifies the analysis. On the other hand, we acknowledge that in reality such a model should be adjusted to take into account various features deviating the result from the theoretical analysis. In case of insurance, such deviation is often modelled with additional loading factors \cite{Marotta2017}, which increases the price to cover insurance expenses, ensures solvency, securing insurance risks, etc. In this paper, we do not consider how much the non-competitive market aspects affect the results of our analysis and leave this issue for future studies. We also would like to underline that other factors (e.g., insurance regulations, deducible, perception of risk, the interdependence of cyber security, etc.)  may affect the results of our study and require specific analysis to estimate the deviation from our core model.
\end{quotation}


\comment Countermeasure independence, both in terms of threat resilience and costs, is also a very strong assumption that will not hold in practice (e.g., a SIEM event monitoring relies on an identity management solution in place, thus their effectiveness against threats is not independent). Finally, the approach assumes that for all considered controls it is possible to estimate a probability for each considered threat scenario occurring with this control implemented. It seems thus that the time investment for an organisation to bootstrap this cost-efficient countermeasure selection process is quite high. 

\reply We discuss the effect of the interdependence of controls on our solution, but leave it for the future work (which is the current work being conducted by our team). 

\begin{quotation}
	\footnotesize
	\newreply In this work, we assumed security controls' costs and probabilities to be independent of each other. In practice, some controls may require installation of others (e.g., security audit may require the presence of monitoring and logging mechanisms) or even conflict with each other (e.g., cryptography may reduce the effectiveness of security audit). Some of these issues can be resolved by pre-processing the input data (e.g., grouping some controls) and others can be resolved by some adjustments in the core algorithms. We leave these steps for future work.
	
	\newreply Last but not least, we admit that our proposal relies on the knowledge of survival probabilities and expected losses, the values which are hard to find. The problem of identifying these values is well-known in the cyber security research and industrial community and is heavily related to the lack of statistical data available for research which is only becoming available \cite{Roman18}. On the other hand, we believe such values can be found by cyber insurers who are collecting data from their customers and are interested to use them for identification of these values. We also may see some real steps in this direction as IBM Security and Ponemon institute's Data Breach report \cite{Ponemon} contains the study (and reports statistics) for the loss estimation depending on the security controls installed.
\end{quotation}


\comment It is stated in Section 5.5 that a company $ " $[...] is most likely to consider a much smaller number of possible controls and be more focused on a small number of relevant threats [...]$ " $ If this would be the case, I am not sure if there is much value in the algorithms proposed, because an exhaustive search implemented in a spreadsheet would work perfectly fine for very small scenarios. So it is larger scenarios that are most interesting for organisations, because then it is hard for them to estimate things quickly. 

A discussion that would systematically review the assumptions, assess what are their practical limitations, and propose some possible alleviations as future research avenues is needed.

\reply We would like to underline that despite using a smaller number of relevant threats and controls (e.g., 10 or 20), the exhaustive search will require significant time, the time grows significantly with every additional number. Our dynamic programming based solutions can do this in manageable time (according to the experiments described in the paper). We underlined the possibility to apply the exhaustive search for very small numbers and have clarified this point in the text as follows:
\begin{quotation}
	\footnotesize
	\newreply
	On the other hand, an organisation thinking about improving its self-protection is most likely to consider a moderate number of possible controls (e.g., 10-20) and be more focused on a moderate number of relevant threats (e.g., 10-20), thus, making application of our DP-based solution acceptable. Naturally, if the numbers are very small, an exhaustive search may be also applicable, but its time of execution grows too fast comparing to dynamic programming based algorithms.
\end{quotation}


\comment Recent SoK paper on cyber insurance in IEEE S\&P 2020 should be included in the literature review (Dambra, Bilge \& Balzarotti "SoK: Cyber Insurance - Technical Challenges and a System Security Roadmap")


\reply We have thoroughly reviewed and highlighted the paper in the both Introduction and Related Work sections.

\comment{Page 4, lines 25-26: "[...] often starting with a basic knapsack problem [17] but also considering specific variation" - please consider rephrasing this sentence, as it is not clear what "specific variation" refers to. Is it "a variation of a knapsack problem"? Is it always the same variation for all cited literature here, or different variations?}

\reply We have rephrased the sentence as follows:

\newreply Several authors \cite{Smeraldi,Sawik,DEWRI,leechoi} focused on formulating the problem of optimising best controls selection where they applied the basic knapsack problem \cite{knapsack}. Even though the main concept is similar, the authors assumed various limitations and modifications of the knapsack problem.

\comment{The basic variables $ x $, $ P $ and $ Loss $ are introduced twice, first on page 5, then on page 6.}

\reply{Thank you for spotting this double definition. We removed the second introduction of these variables.}

\comment Page 7, line 31: It is not clear, why we are talking about successful penetration into a system here because cyber threats can be of different nature. More generically, this can be a probability that the threat scenario occurs given countermeasures in place. 

\reply The sentence have been re-worded to keep the more generic meaning as follows:	
\begin{quotation}The probability of threat $i$ successfully passing through all installed security controls is denoted as $p^{i}(K_s)$, which eventually can be seen as a vector for all $n_t$ threats, $ \vec{p}(K_s) = \langle p^1(K_s), ~p^2(K_s), ..., ~p^{n_t}(K_s) \rangle $.
\end{quotation} 

\comment Also, it is not really clear at this point, why we are speaking here (and in Eq. 4) about the optimal solution $ K_s|x $, and not a generic set $ K_s $.


\reply We have revised the section and made it clear to understand. $ K_s|x $ is introduced later in the section when it is required.

\comment{Page 8, Equation 5: It is not clear, why both $ F $ and $ Z $ are used in this equation. $ F $ is already a set of threat scenario frequencies that is expected by an organization (I presume, over a specific period of time). Why there is another variable $ z $ that also represents an amount of threats over a period of time (i.e., possible frequencies). According to line 46 on page 7, $ F $ is expected threat frequencies, because this is what the insurer wants to consider. Why there is a need to consider all possible threat scenario occurrences if there is already expected threat frequencies available?}


\reply We have revised the section and re-structured it in a way that readers easily understand the concept. Although the variables may relate to each other, we cannot use only one of them (e.g., $F$), since for rigorous transformation (as it is defined in the article) we need to extract $z$-s out of the utility function (or push the relevant probabilities under it). Since this is not possible, we are constrained to use both of these parameters. \\
We have clarified the difference between $ F $ and $ Z $ in Section 3. Moreover, we hope that the new structure and gradual introduction of variables (and increasing complexity) in Section 3 will help the reader to understand the computations better.

\comment{Also, I cannot interpret the index $ i $ in $ p_i $ in Equation 5. What does it range over? I note that this index is present also in Eq. 6, but it is gone in Eq.7 when the expectation is computed.}


\reply{We fixed the issue and further used a proper notation for the vector.}

\comment{Page 8, the final sentence of Section 3.1 is not clear to me. Which "models described above [...] are found to be valid" are referred to here? Models in this section, or in the related literature?}


\reply We made it explicit as the following: 

\newreply Thus, our further contribution could be applied if one of the conditions (Equations \ref{eq:MaxSecond} and \ref{eq:MaxThird}) described above is found to be valid.

\comment{Figure 5 is hard to read in a printed copy. I would suggest to increase the font size.}


\reply{We increased the font and hopefully made it much clearer to see.}


\comment{Some references have a strange style for authors' names: "Surname\_1, Name\_1, Name\_2 Surname\_2, and Name\_3 Surname\_3". E.g., [4, 5, 6, 10], etc.}


\reply{We fixed the issues.}


\comment{Typos:\\
	Page 4, line 26: The word $ " $problems$ " $ appears twice. It should be "problem" in fact, and there is no space before the reference [17].\\
	Page 4, lines 47-48: "[...] we propose our exact algorithmic solution [...] and adapted it for [...]" - some issue with tenses here.\\
	Page 6, line 46: "that is not needed here.\\
	Page 16, line 16: "[...] used optimisation solutions [...]" - perhaps, "optimisation techniques/approaches" is better here.\\
	Page 16, line 49: "[...] and check if" - should be "checks".\\
	Page 18, line 10: "Windows 10 operational system" - should be "operating system".}

\reply{We fixed above-mentioned typos and other mistakes in the paper.}


\reviewer
%\newperson{Reviewer 2}{R2}

\comment The text is well written. There are a few points to correct as punctuation.

\reply We proofread the paper and did our best to correct the language and punctuation errors.

\comment The general goal can be more detailed to include how the goal will be achieved.

\reply We have revised the section and added the paragraph written below to describe how the goal can be achieved. We have further added a systematic discussion section on the assumptions we took and future directions (see Section~\ref{sec:MAinDiscussion}).

\begin{quotation}
	\footnotesize
	\newreply The theoretical analysis is based on the utility theory and assumes a competitive insurance market in place. The resulting optimisation problem is represented as a multi-objective knapsack problem where minimisation of risks for every threat is a separate objective. The algorithmic solutions for the problem are based on the dynamic programming \cite{bazgan}. Moreover, we enhance the algorithm by applying our projection idea and compare the results by conducting several experiments.
\end{quotation}


\comment The related work and other references are actual and I'm not capable to perceive some omission. The authors made discussions about them and comparisons with the proposed work.

\reply Thanks for the comment. We have further revised the section and added some papers suggested by RA.

==> 00_Reply1.tex <==
% In the preamble
%%%%%%%%%%%%%%%%%%%
\def\boxedreviewnote#1{\fbox{#1}}

\usepackage{xcolor}

\definecolor{darkred}{rgb}{0.8,0,0}

% Comment the following to get version without comments

\newcommand{\fixed}[1]{{\color{darkred}#1}}

\def\reviewnote#1{\marginpar{#1}}


\newcounter{reviewer}

\renewcommand{\thereviewer}{\Alph{reviewer}}

\newcounter{comment}[reviewer]

\def\editor{\section*{\dotfill\textsc{Comments from Meta-review }\dotfill}}

\def\reviewer{\refstepcounter{reviewer}\section*{\dotfill\textsc{Comments from Reviewer }\thereviewer\dotfill}}

\def\comment{\refstepcounter{comment}\subsection*{\textsc{Comment} \thereviewer.\thecomment}\ignorespaces}%\vspace{-0.5\baselineskip}}

%\def\reply{\vspace{-0.5\baselineskip}\subsubsection*{\textbf{Reply}}}

\def\reply{\vspace{0.5\baselineskip}\par\noindent\textbf{Reply:}\ignorespaces~\hangindent 7ex}

\def\newreply{\vspace{0.5\baselineskip}\par\noindent\hspace*{6ex}\ignorespaces~\hangindent 7ex}

%\vspace{-0.5\baselineskip}}

%\def\added{\textsc{\bf{Added text:}}\\}

%%%%%%%%%%%%%%%%%%%%%%

%\let\mylabel\label

%\def\label#1{\protect\expandafter\mylabel{#1}\protect\fbox{#1}}

%%%%%%%%%%%%%%%%%%%%%%%%



%%%%% In the text




%%%%%%%%%%%%%%%%%%%%%%%

\reviewer \label{r1}

\comment This paper focuses on formalizing existing knowledge of

the visible process of data sharing into a logical framework.

They provide a calculus based on intuitionistic quantifier-free

first-order logic which also contains custom inference rules regarding

known tracking behavior. Such an approach can be used by different

websites and advertisers to identify whether they need to comply

with relevant privacy regulations regarding PII collection. In

addition, one can verify different claims about tracking behavior

through the use of automated theorem provers. The authors also use

their logical framework to evaluate the effectiveness of different

privacy-enhancing technologies that are able to mitigate unintended

user tracking in the Alexa Top 100 websites based on data obtained

from the openWPM dataset.



Strengths:

\begin{itemize}
	
	\item The paper is in general well written and easy to follow. It also does a commendable job in being self-contained regarding different aspects of the problem and their techniques.
	
	\item The formal part of the work performed by the authors is solid and makes sense.
	
	\item An impressive amount of work has gone into this paper.
	
	\item The authors have done a commendable job in scoping the problem in the sense that it is clear what is included in their formal model and what is excluded. 
	
\end{itemize}



Weaknesses:

\begin{itemize}
	
	\item The main criticism I have about the work is that the authors did not
	
	do a thorough job in motivating the problem and discussing different
	
	aspects of the problem in details (e.g., intended users, usability,
	
	extension, scalability, generality).
	
\end{itemize}



\reply Thank you for your comments. We hope we have addressed your concerns

as we detail in the following answers.



\comment \label{r1:update:motivation}

The authors did not sufficiently motivate the need for formalizing the

known tracking behavior of the Internet. It seems the authors are formalizing

what is already known in the literature. What is the added value of this

formalisms? Are there atomic, ground predicates the framework can derive

which is hard to derive manually? Did the authors find such surprising

results? Is transitivity of data sharing the only sort of complications

in inferring facts? For instance, if x shares data with A, A then shares

it with B, and B then shares it with C, then one can derive that x's data

can be possessed by C.





\reply We indeed formalized the current techniques employed for tracking (as our goal is not to develop a new detection mechanism or analyze new techniques as showed in Tab.~\ref{tab:PaperComparison}).



\newreply The added value of the formalization stays in the ability to provide an explanation, in the form of a proof, to show tracking practices and that can help users in determine e.g. the adds-on to install or if certain websites should comply to COPPA due to interaction with children-related websites. We have added a paragraph (\emph{Goal}) in Section\S\ref{sec:introduction} to underline the added value of this framework. We further discussed the added value in an appropriate section (Section\S\ref{sec:scalability}).



\comment \label{r1:update:utility}

The possible utilities of their framework are scattered all

over the paper. I sincerely think that having it one place could drive

home the point easily. Also, such interesting and non-trivial finding

could motivate the use of such a framework.

==> 02_ProblemSpecification.tex <==
\section{Problem specification}
\label{sec:Prob}
%The main goal of this work is the development of a mathematical and algorithmic framework to help a risk-averse organization to select cost-effective security controls to be implemented which guarantee a rational distribution of security expenditure between self-protection and cyber insurance.

%In the cyber insurance and cyber security economics literature, risk is often considered having in mind only one threat \cite{Bohme-L,Ogut2004}. This significantly simplifies the analysis and makes the possible application of efficient mathematical solutions. On the other hand, in practice, organisations face a number of cyber threats of a different kind which may cause different losses (e.g., see examples of threats from the ISO27005 standard \cite{ISO27005}). This makes impossible direct application of theoretical findings in reality since considering each threat separately does not allow conducting a holistic analysis.

%Cyber insurance literature usually assumes that knowing investment in self-protection is possible to determine the probability of a threat occurrence \cite{Marotta2017,Anderson}. In practices, it is required to tell what security controls should be installed in order to obtain the highest level of protection. Moreover, some security controls could be already pre-installed (i.e., some amount of investment could be already spent and its current distribution could be not cost-efficient). Moreover, various legal, contractual and organisational obligations could force installing not the most cost-effective security controls. In this case, it is not enough to consider only the amount of investments, but it is required to determine the best additional improvement of security having in mind existing (probably, not cost-efficient) security configuration.

%In general, once an organisation has assessed its risks, it has four basic options to deal with these risks. \emph{Risk avoidance} suggests refraining from conducting a risky business. \emph{Risk transfer} (e.g., insurance) proposes transferring risk to other organisation (e.g., insurer) for some fee (called the premium). \emph{Risk mitigation} helps to reduce the risk by the implementation of additional security controls. Finally, \emph{risk acceptance} simply tells that the organisation should be prepared to pay for the possible risk occurrences itself (knowingly or unknowingly). 

Consider a generic case, in which an organisation looks for the most cost-efficient way to treat its cyber risks. It decides to invest $x$ to improve its security controls and pay $P$ as a premium for some insurance coverage. Regardless of the investments and insurance it still may face some residual losses. If the organisation has $W^0$ as an initial wealth (or expected benefit from its core business), then it may expect the following wealth $\boldsymbol{W}$ in the future:
\begin{align}
\boldsymbol{W}=W^{0}-P-\boldsymbol{Loss}-x
\label{eq:Basic}
\end{align}
Since we are predicting the future wealth ($\boldsymbol{W}$), $\boldsymbol{Loss}$ is a random variable\footnote{The random values are written in bold.}, i.e., a variable which may take different values (e.g., 0 if no threat occurs, or some $L$ if the threat occurs and causes damage) with some probability. 

Equation~\ref{eq:Basic} must always be greater than 0, otherwise, the organisation should not engage in this business (risk avoidance). Finally, $\boldsymbol{Loss}$ is the residual risk for the organisation to bear. In short, Equation~\ref{eq:Basic} takes into account all risk treatment options, although some of them could be found not necessary (i.e., equal to 0), and shows how different options affect the final wealth. Naturally, a rational organisation should aim for maximising it's $\boldsymbol{W}$. 

\emph{Our goal in this article is to find the efficient distribution of investments, i.e., self-investments, insurance and accepted risk. Furthermore, we go further and explicitly show how these investments should be used by selecting the best set of security countermeasures to achieve this efficient budget distribution.} Considering the efficient distribution of investments and selection of controls helps us to achieve the desired cost-effectiveness, in contrast to efficient threat mitigation only considered in many of the related works \cite{ANDREW1,Smeraldi,Sawik,DEWRI}.

In the following of this section, we will define the problem in details and explicitly show how security countermeasures affect the Equation~\ref{eq:Basic}. The main parameters used in this paper are listed in Table~\ref{tab:Notat}.
%\subsection{Problem statement without Cyber insurance available}

\begin{table*}[!t]
	\begin{center}    
		\resizebox{1\textwidth}{!}{
			\footnotesize
			\begin{tabular}{| c  l | c  l |}
				\hline
				$W^0$ & - initial wealth & $ \bar{\pi} $ & - probability of a threat \textit{survival}\\
				\hline
				$x$ & - security investment & $ \bar{F} $ & - expected number of threat \textit{attempts}     \\
				\hline
				$  c $ & - cost of a countermeasure & $\bar{p}$ & - probability of a threat \textit{occurrence}\\    
				\hline
				$P$ & - premium & $\bar{z}$ & - \textit{number} of threat occurrences \\
				\hline 
				$ K $ & - a set of \textit{available} countermeasures & $ \bar{L} $ & - loss    \\
				\hline
				$ K_s $ & - a set of \textit{selected} countermeasures & $\bar{I}$ & - indemnity     \\
				\hline
			\end{tabular}
		}
	\end{center}
	\caption{Notations adopted in this work}
	\label{tab:Notat}
\end{table*}

\subsection{Formal model}
Let us take into a consideration \textcolor{blue}{that} an organisation which has conducted risk identification phase of risk assessment and has identified $ n_t (n_t \in \mathbb{N}^+) $ relevant threats. For each threat, a corresponding expected loss has been defined $ \bar{L} = \langle L^1, L^2, ..., L^{n_t} \rangle $, where $\bar{L}$ is a vector and $L^i (1 \leq i \leq n_t) $ is its i-th member.

If an organisation buys insurance, it pays some premium regularly and expects some coverage of a loss if a threat occurs (called indemnity $ \bar{I}$). Indemnity is also a vector of size $n_t$, since depending on the insurance product bought, different threats may get different coverage, but the coverage is always lower than the loss itself ($\forall i,~I_i<L_i$). Thus, we may identify two situations: if no threat occurs ($\boldsymbol{Loss}=0$) or if a threat occurs (and $\boldsymbol{Loss}=L_i-I_i$):
\begin{align}
W^{nt} = W^0 - x - P &~~~~~~~if~no~threats~occur\nonumber \\
W^t = W^0 - x - P - L_i + I_i &~~~~~~~with~~threat~i~occurred
\label{Wealth}
\end{align}  

Investments will be spent for installation and application of a set of security controls $K_s$, which can be seen as a subset of the set of all possible security controls $K$ (e.g., the ones that could be found in ISO27002 \cite{ISO} or NIST 800-53 \cite{NIST800}). Considering the case, the interplay of investment $x$ and set of controls $K_s$ should be assumed at management level. Let the cost of a countermeasure be a function and its result be a finite non-negative value $c:K\mapsto \mathbb{N}^{+}$. The overall cost of installed countermeasures $K_{s}\subseteq K$ ($c({K_{s}})$) is, naturally, computed as: 
\begin{align} c({K_{s}}) = \sum_{\forall k\in K_{s}} c(k). \end{align}
Since in the paper we are interested in identification of countermeasures, we use the following notation $K_s|x$ to say that a set $K_s$ is the most effective set of countermeasures which can be selected with the maximal cost $x$ (i.e., $c({K_{s}})\leq x$). 
%The lower index ($i$) for investments and the set of selected security controls is used in order to compare various investments and similar sets.

The probability of successful penetration into the system investing $x$ into its protection, $ p $ is also a vector ($ \bar{p}(K_s|x) = \langle p_1(K_s|x), ~p_2(K_s|x), ..., ~p_{n_t}(K_s|x) \rangle $). Now, if we know the frequency of threat occurrence  $ \bar{F} = \langle F^1, F^2, ..., F^{n_t} \rangle $, the overall risk for the organisation can be found as follows.
\begin{align}
Risk (K_s|x, \bar{L}) = (\bar{F}\cdot\bar{p}(K_s|x))\times\bar{L},
\label{OverAllRisk}
\end{align}
where $\bar{a} \times \bar{b}$ is a usual matrix multiplication of two vectors given as $ \bar{a} \times \bar{b} \rightarrow \sum_{j=1}^{n_t} a^j * b^j $ and Hadamard product of two vectors $ \bar{a} $ and $ \bar{b} $ is a vector $ \bar{c} = \bar{a} \cdot \bar{b} = \langle a^{1}*b^{1},a^{2}*b^{2},...,a^{n_{t}}*b^{n_{t}}\rangle $. In this paper, we avoid transposition of vectors, required for proper representation of matrix multiplication, to simplify the formalisation since this precision is not crucial for understanding of the paper. 

In cyber insurance, a premium is usually computed through the estimated risk. A usual assumption is to consider a competitive insurance market \cite{Marotta2017} for which the premium is equal to risk for the insurer (i.e., $P=Risk (K_s|x, \bar{I}))$.

Since a threat may occur more times than once in an observed period, and harm the organisation more than once, we need to take into account distribution of probabilities with respect to the number of threat occurrences. Let $ \bar{z} = \langle z^1, z^2, ..., z^{n_t} \rangle $ be a random vector of numbers of threat occurrences (one per threat) and $p(\bar{z}|K_{s},x)$ be the probability that the considered organization will face $\bar{z}$ incidents for some period of time under the condition that investments in self-protection are $x$ and implemented countermeasures are $K_{s}$\footnote{We write $\bar{z}|K_{s},x$ instead of $\bar{z}|(K_{s}|x)$ for clarity.}. Also, $ \bar{F}\cdot\bar{p}(K_{s}|x)=\sum_{\forall \bar{z}}p(\bar{z}|K_{s},x)\cdot \bar{z}$. In short, it is not enough to define ``no threat'' and ``threat occurred'' states for taking into account all possible wealth values $W$, but also consider different amount of occurred threats. Thus, the wealth for some specific amount of threats $\bar{z}$ can be defined as:
\begin{align}
&W(\bar{z},K_{s},x,\bar{I})=W^0-(\bar{F}\cdot\bar{p}(K_{s}|x))\times \bar{I}-x-\bar{z}\times(\bar{L}-\bar{I}), \\
&where~ \bar{I}-\bar{L}=\langle I^{1}-L^{1},I^{2}-L^{2},...,I^{n_{t}}-L^{n_{t}}\rangle. \nonumber
\end{align}

Similar to other economic models \cite{Marotta2017,Ogut2004,Ehrlich1992}, we assume an organisation to be risk-averse and use utility of possessing a certain amount of wealth ($U(W)$) instead of the wealth $W$ itself. The utility function is considered to be continuous, non-decreasing, and concave, i.e., $U'(W)>0$ and $U''(W)<0$.
\begin{align}
&U(W(\bar{z},x,\bar{I}, K_{s}))=U(W^0-(\bar{F}\cdot\bar{p}(K_{s}|x))\times \bar{I}-x-\bar{z}\times(\bar{L}-\bar{I})).\label{eq:utility} 
\end{align} 
Finally, the expected utility is equal to:
\begin{align}
& E[U]= \sum_{\forall \bar{z}}p(\bar{z}|K_{s},x)U(W^0-(\bar{F}\cdot\bar{p}(K_{s}|x))\times \bar{I}-x+\bar{z}\times(\bar{I}-\bar{L})). \label{eq:ExpectedUtility} 
\end{align}
Our goal transforms into maximisation of the expected utility ($E[U]$) by selecting the optimal $x$, $\bar{I}$ and $K_{s}$. 

In these settings, it is possible to prove that the optimal $\bar{I}$ for an organisation is equal to $\bar{L}$ (see the proof in the Appendix~\ref{sec:Indemnity}). In other words, a risk-averse organisation insures all risks left after reduction if insurance option is available. This allows us to reduce Equation~\ref{eq:ExpectedUtility} to: 
\begin{align}
\max\limits_{x, K_{s}}U(W^0-x -(\bar{F}\cdot \bar{p}(K_{s}|x))\times\bar{L}). \label{eq:MaxSecond}
\end{align}
Since the utility function is non-decreasing, we need to maximise its argument, or simply minimise the following part, which we call \emph{expenditure} in the following:
\begin{align}
\min\limits_{x, K_{s}} (x +(\bar{F}\cdot \bar{p}(K_{s}|x))\times\bar{L}). \label{eq:MaxThird}
\end{align}

At this point we need to note, that our problem becomes equivalent to a risk-neutral approach (i.e., if $U(W)=W$) for selecting security budget distribution and controls selection if no insurance is available (in this case, the premium becomes the accepted residual risk). The organisation should simply minimise its investments in self-protection and residual risk. Thus, our further contribution could be applied if one of the \textcolor{blue}{conditions} (Equations \ref{eq:MaxSecond} and \ref{eq:MaxThird}) described above is found to be valid.

\subsection{Detailed problem specification}
In order to minimise Equation~\ref{eq:MaxThird}, we need to compute $p(K_{s}|x)$ and determine the procedure for selection of $K_s$ in a way to minimise this component and ensure that we do this with investments less or equal to $x$. 

Let $ \pi^{j}(k) \in [0;1]$ be the probability that a threat $j$ passes through (survives) control $ k \in K_{s} $; control $k$ completely eliminates threat $j$ if $\pi^{j}(k) = 0$, and is entirely powerless against the threat if $ \pi^{j}(k) = 1 $. Let $\bar{\pi}(k)$ be a vector of all probabilities of survival if control $k$ is installed, and the overall probability of survival can be computed as\footnote{We assume effects of controls to be independent from each other.}:
%
\begin{align} \bar{\pi}({K_{s}}) = \prod_{\forall k\in K_{s}} \bar{\pi}(k),  \label{eq:OverallProb}
\end{align}
where $\prod_{\forall k\in K_{s}}$ stands for the Hadamard product.


Now, we are able to connect $\bar{\pi}({K_{s}})$ and $\bar{p}(K_{s}|x)$. We say that  $\bar{p}(K_{s}|x)=\bar{\pi}({K_{s}})$ if $K_{s}$ minimises Equation~\ref{eq:MaxThird} and its overall cost is below $x$:
\begin{align} 
\min\limits_{\forall K_{s}\subset K} (\bar{F}\cdot \left[ \prod_{\forall k\in K_{s}} \bar{\pi}(k)\right])\times \bar{L}+x~~~and~~~
\sum_{\forall k\in K_{s}} c(k) \leq x \label{eq:Cond}.
\end{align}
Equation~\ref{eq:Cond} is the core problem we are tackling with in this paper. 

==> Additional.tex <==
\begin{algorithm}[!th]
	\caption{Selecting the best set of countermeasures}\label{alg:main}
	\begin{algorithmic}[1]
		\Procedure{searchForOptimalInvesments}{$K$, $C$, $ \pi $, $\bar{R}$, $x_{limit}$}
		\Require $K$ \Comment{- a set of countermeasures}\\
		$c:K\mapsto \mathbb{N}$ \Comment{- cost function}\\
		$\pi:K\mapsto 2^{[0;1]}$ \Comment{- survival probability per threat function}\\
		$\bar{R}$ \Comment{- current Risk vector of $\mathbb{N}^{+}$ values}\\
		$x_{init}\in \mathbb{N}$ \Comment {- Investment Limit (optionally)}\\
		$C\in \mathbb{N}$ \Comment{the greatest common divisor for countermeasure cost}
		\Ensure \texttt{lowest $(\prod \pi(K_{i}|x))\times \bar{R} + x$ for optimal security investment $ x^* $ or within a given $ x $}
		\BState \emph{\textbf{Main Function}}:
		\Require ID of the countermeasure
		\State Call Initial Population Function
		\State Main Loop:
		\State: Crossover process:
		\State: Mutation process:
		\State: Run the loop for \textit{LIMIT}:
			\end{algorithmic}
		\begin{algorithmic}[1]
		\BState \emph{\textbf{Initial Population}}:
		\State Initialize the population of N number by removing ones that do not satisfy the following condition
		\State $ Perc = 100 $
		\For {i:=1 to N} \Comment N $ \rightarrow $ maximum number of chromosomes
		\State Generate Random Chromosome \Comment select only one countermeasure in the chromosome ensuring the best one if there are more than two countermeasures which have the same ID.
		\State Set all genes of chromosome as 0
		\State Replace the $ Perc $ percentage of them as 1
		\If {($x_{limit}$ $ > 0 $ \&\& $x_{limit}$ $ < U $)} 
		\State $ i:= i - 1 $ \Comment Remove the chromosome which does not satisfy/survive the condition
		\State $ Perc:= Perc - 1 $ \Comment Decrease the percentage of replacement
		\EndIf
		\EndFor \\
		\Return Generated Random Chromosomes
			\end{algorithmic}
		\begin{algorithmic}[1]
				\BState \emph{\textbf{Crossover:}}
		\State Make crossover between a randomly chosen chromosome and our selected chromosome by changing the half of them.
		
		\Require Current Chromosomes
		\For {i:=1 to N} \Comment N $ \rightarrow $ N: Number of current chromosomes
		\State j = rand(1, N) $ \rightarrow $ generate random number in range 1 to N
		\State nextGen = crossover i-th and j-th chromosome \Comment i-th chromosome's first half and j-th chromosome's second half genes
		\EndFor
		\State Call the Merge function (current and nextGen chromosomes)\\
		\Return Merged Chromosomes
		\BState \emph{\textbf{Mutation:}} \Comment Mutate the chromosomes for a given number of bits/genes
		\Require k
		\For {i:=1 to N} \Comment N $ \rightarrow $ N: Number of current chromosomes
		\State Replace the k number of random bits in the chromosome
		\State nextGen = mutated i-th chromosome	
		\EndFor
		\State Call the Merge function (current and nextGen chromosomes)\\
		\Return Merged Chromosomes
		\BState \emph{\textbf{Merge Function}}:
		\Require Current chromosomes, nextGen chromosomes
		\State \textbf{Append} Current chromosomes \textbf{to} nextGen chromosomes \Comment merge the two lists of chromosomes
		\State \textit{weight} = $(p(K_{i}|x))\times \bar{R} + x$
		\State \textbf{Sort} Current chromosomes by their \textit{weight} \Comment z to a way is used to sort the chromosomes 
		\State Select 60\% of chromosomes as good and rest as a random
		\EndProcedure
	\end{algorithmic}
\end{algorithm}












\begin{algorithm}[!th]
	\caption{Main Function of the GA algorithm}\label{alg:MainFuncs}
	\begin{algorithmic}[1]
		\Procedure{MainFunction}{$K$, $c$, $ \pi $, $\bar{R}$, $x_{limit}$, $ b $, $ LIMIT $, $ {Perc} $}
		\Require 
		$K$ \Comment{- a set of countermeasures}\\
		$c:K\mapsto \mathbb{N}$ \Comment{- cost function}\\
		$\pi:K\mapsto 2^{[0;1]}$ \Comment{- survival probability per threat function}\\
		$\bar{R}$ \Comment{- current risk vector of $\mathbb{N}^{+}$ values}\\
		$x_{limit}\in \mathbb{N}$ \Comment {- investment limit}\\
		$b \in \mathbb{N}$ \Comment {- a unique number assigned to each countermeasures}\\
		$LIMIT \in \mathbb{N}$ \Comment {- a constant value to run the GA}\\
		$Perc \in \mathbb{N}$ \Comment {- Percentage}
		\Ensure \texttt{lowest $(\prod \pi(K_{i}|x))\times \bar{R} + x|x_{limit}$ } \Comment for optimal security investment $ x $ or within a given $ x_{limit} $
		\BState \emph{\textbf{Check the inputs}}:
		\State Return acknowledgement message
		\BState \emph{\textbf{Call Initial Population Function}}:
		\BState \emph{\textbf{New Population}}: $ \rightarrow $ Loop for \textit{LIMIT}:
		\State Crossover process:
		\State Mutation process:
		\State Merge process:
		\EndProcedure
	\end{algorithmic}
\end{algorithm}



\\
\begin{algorithm}[!th]
	\caption{Initial Population and Fitness Assignment of the GA algorithm}\label{alg:Init1}
	\begin{algorithmic}[1]
		\Procedure{InitialPopulation}{$K$, $c$, $ \pi $, $\bar{R}$, $x_{limit}$, $ b $, $ LIMIT $, $ {Perc} $}
		\State $ Perc = 100 $
		\For {i:=1 to N} \Comment N $ \rightarrow $ maximum number of chromosomes
		\State Generate Random Chromosome
		\If {$ b > 0 $}
		\State Select a better chromosome among the same ID countermeasures
		\EndIf
		\State Set all genes of chromosome as 0
		\State Replace the $ Perc $ percentage of them as 1
		\If {($x_{limit}$ $ > 0 $ \&\& $x_{limit}$ $ < U $)} 
		\State $ i:= i - 1 $ \Comment Remove the chromosome which does not satisfy/survive the condition
		\State $ Perc:= Perc - 1 $ \Comment Decrease the percentage of replacement
		\EndIf
		\EndFor \\
		\Return Generated Random Chromosomes
		\EndProcedure
	\end{algorithmic}
\end{algorithm}


\begin{algorithm}[!th]
	\caption{Creation of New Population}\label{alg:NewPop}
	\begin{algorithmic}[1]
		\Procedure{NewPopulation}{$K$, $c$, $ \pi $, $\bar{R}$, $x_{limit}$, $ b $, $ LIMIT $, $ {Perc} $, $N$, $e$}
		\BState \emph{\textbf{Crossover:}}
		\State Make crossover between a randomly chosen chromosome and our selected chromosome by changing the half of them.
		
		\Require Current Chromosomes
		\For {i:=1 to N} \Comment N $ \rightarrow $ N: Number of current chromosomes
		\State j = rand(1, N) $ \rightarrow $ generate random number in range 1 to N
		\State nextGen = crossover i-th and j-th chromosome \Comment i-th chromosome's first half and j-th chromosome's second half genes
		\EndFor
		\State Call the Merge function (current and nextGen chromosomes)\\
		\Return Merged Chromosomes
		\BState \emph{\textbf{Mutation:}} \Comment Mutate the chromosomes for a given number of bits/genes
		\Require e
		\For {i:=1 to N} \Comment N $ \rightarrow $ N: Number of current chromosomes
		\State Replace the k number of random bits in the chromosome
		\State nextGen = mutated i-th chromosome	
		\EndFor
		\State Call the Merge function (current and nextGen chromosomes)\\
		\Return Merged Chromosomes
		\BState \emph{\textbf{Merge Function}}:
		\Require Current chromosomes, nextGen chromosomes
		\State \textbf{Append} Current chromosomes \textbf{to} nextGen chromosomes \Comment merge the two lists of chromosomes
		\State \textit{weight} = $(p(K_{i}|x))\times \bar{R} + x$
		\State \textbf{Sort} Current chromosomes by their \textit{weight} \Comment z to a way is used to sort the chromosomes 
		\State Select 60\% of chromosomes as good and rest as a random
		\EndProcedure
	\end{algorithmic}
\end{algorithm}






\begin{algorithm}[!th]
	\caption{Selecting the best set of countermeasures}\label{alg:main1}
	\begin{algorithmic}[1]
		\Procedure{searchForOptimalInvesments}{$K$, $c$, $\pi$, $\bar{F}$, $\bar{L}$, $x_{init}$, $pr_{init}$, C}
		\Require $K$ \Comment{- a set of countermeasures}\\
		$c:K\mapsto \mathbb{N}$ \Comment{- cost function}\\
		$\pi:K\mapsto 2^{[0;1]}$ \Comment{- survival probability per threat function}\\
		$\bar{F}
		$ \Comment{- frequency vector of $\mathbb{R}^{+}$ values}\\
		$\bar{L}$ \Comment{- single loss expectency vector of $\mathbb{N}^{+}$ values}\\
		$x_{init}\in \mathbb{N}$ \Comment {- initial investments}\\
		$\bar{pr}_{init}$ \Comment{- initial overall probability of survival vector of values from $[0;1]$} \label{line:LastDefinition}\\
		$C\in \mathbb{N}$ \Comment{the greatest common divisor for countermeasure cost}
		\Ensure \texttt{lowest $(\bar{F}\cdot \bar{pr}(K_{i}|x))\times \bar{L} + x$ for optimal security investment $ x^* $}
		\State $ exp \Leftarrow (\bar{F}\cdot\bar{pr}_{init})\times\bar{L} + x_{init}$  \Comment{Remember the initial expenditure as optimal} \label{line:firstA}
		\State $P^{*}_{min}=\bar{F}\cdot \left[ \prod_{\forall k\in K} \bar{\pi}(k)\right])\times \bar{L}$
		\State $ x^* \Leftarrow 0 $ \Comment{Optimal Investment starts with $x_{init}$} 
		\State $\forall j~T[j][0] \Leftarrow~\{\bar{pr}_{init}\}$ \Comment{a dynamic matrix of optimal probabilities. Add new (and the first) column $x=x_{init}$, with just one vector $\bar{pr}_{init}$} \label{line:Tinit}
		\State $ x \Leftarrow C $ \label{line:xinit} \Comment{the size of set $K$}
		\State $ n_{k} \Leftarrow |K| $ \label{line:finInit}
		\While{$x+x_{init}  \le exp-P^{*}_{min} $} \Comment{Do while $x$ is below the optimal expenditure} \label{line:While}
		\State $\forall j~T[j][x] \Leftarrow~\{\bar{pr}_{init}\}$ \Comment{Add new column x, initialised with vector $\bar{pr}_{init}$}
		\For{$j \Leftarrow 1, n_{k}$} \Comment{for all countermeasures} \label{line:For}
		\If{($c(k_j)$ $\leq$ $x$ )} \label{line:CompareCost} \Comment{check the cost limit}
		\State $ T[j][x] \Leftarrow non-dominant 
		\left\{ 
		\begin{array}{l}
		\bigcup\limits_{\forall l} \bar{\pi}(k_j) \cdot T[j-1][x-c(k_j)][l]\\
		T[j-1][x] 
		\end{array}
		\right.$ \Comment{store all non-dominant vectors comparing two sets: with new control and without.} \label{line:Selection}
		\Else
		\State $T[j][x] \Leftarrow T[j-1][x]$ \Comment{continue without adding new control $j$ } \label{line:HighCost}
		\EndIf    
		\EndFor
		\For{$l\Leftarrow 0,|T[n_{k}][x]|$} \Comment{for all vectors stored in $T[n_{k}][x]$}
		\If{$ (\bar{F}\cdot T[n_{k}][x][l])\times \bar{L} + x + x_{init}  < exp $} \Comment{reduced the expenditure?} \label{line:CheckCondition}
		\State $ exp \Leftarrow \bar{F}\cdot T[n_{k}][x][l])\times \bar{L} + x + x_{init} $ \Comment{Store this expenditure as optimal} \label{line:reSetCondition}
		\State $x^* \Leftarrow x$ \Comment{Remember these investments as optimal} \label{line:reSetOptimal}
		\EndIf
		\EndFor
		\State $ x \Leftarrow x + C $
		\EndWhile\\
		\Return [$ exp, x^*$]
		\EndProcedure
	\end{algorithmic}
\end{algorithm}
